Tight Mobile Byzantine Tolerant Atomic Storage

This paper proposes the first implementation of an atomic storage tolerant to mobile Byzantine agents. Our implementation is designed for the round-based synchronous model where the set of Byzantine nodes changes from round to round. In this model we explore the feasibility of multi-writer multi-reader atomic register prone to various mobile Byzantine behaviors. We prove upper and lower bounds for solving the atomic storage in all the explored models. Our results, significantly different from the static case, advocate for a deeper study of the main building blocks of distributed computing while the system is prone to mobile Byzantine failures.

==> algoFree.tex <==
% !TEX root = main.tex


In this section we present a protocol emulating the behavior of a SWMR Regular register.

We will prove in the following that it requires $n \ge 3f+1$ under the Garay's MB model and $n \ge 4f+1$ under the extended MB model.


%==============================================================================

\begin{figure}[ht]
\centering
%	\subfigure[Write Protocol: client side]{
\fbox{
\begin{minipage}{0.4\textwidth}
%\footnotesize
\scriptsize
%\renewcommand{\baselinestretch}{2.5}
\resetline
\begin{tabbing}
aaaA\=aA\=aA\=aaaA\kill

{\bf Init}: ~~ \\

\line{I-} \> $val_i \leftarrow \bot$;\\

\line{I-} \> $sn_i \leftarrow 0$;\\

%\line{I-} \> $last\_writer_i \leftarrow \bot$;\\

\line{I-} \> $old\_val_i \leftarrow \bot$;\\

\line{I-} \> $old\_sn_i \leftarrow -1$;\\

%\line{I-} \> $old\_writer_i \leftarrow \bot$;\\

\line{I-} \> $cured_i \leftarrow {\sf false}$;\\

\line{I-} \> $update_i \leftarrow \emptyset$;\\

~---------------------------------------------------------------------------------------------------------------\\

{\bf every} $\Delta$ time units {\bf do}:\\

\line{M-} \> $update_i \leftarrow \emptyset$;\\

\line{M-} \> {\bf if} \= $(\neg cured_i)$\\

\line{M-} \> \> {\bf then} \= ${\sf broadcast}$ {\sc echo}$(i, <val_i, sn_i old\_val_i, old\_sn_i>)$;\\

\line{M-} \> \> {\bf else} \= $val_i \leftarrow \bot$;\\

\line{M-} \> \> \> $sn_i \leftarrow 0$;\\

\line{M-} \> \> \> $old\_val_i \leftarrow \bot$;\\

\line{M-} \> \> \> $old\_sn_i \leftarrow -1$;\\

\line{M-} \> {\bf endif}\\
%~\\

~---------------------------------------------------------------------------------------------------------------\\

{\bf when} \=  {\sc echo} $(j, <val, sn, oval, osn>)$ \= is  ${\sf received}$: \\ 

\line{M-} \> {\bf if} \= $(\nexists <j, -, -> \in update_i)$\\

\line{M-} \> \> {\bf then} \= $update_i \leftarrow <j, val, sn>$;\\

\line{M-} \> \> \> $update_i \leftarrow <j, oval, osn>$;\\

\line{M-} \> \> {\bf else} \= $\forall <j, -, -> \in update_i : update_i \leftarrow update_i \setminus <j, -, ->$;\\

\line{M-} \> {\bf endif}\\

~---------------------------------------------------------------------------------------------------------------\\

{\bf when} \=  $\exists <-, val, sn> \in udate_i$ \= occurring at least $f+1$ times: \\ 

\line{M-} \> {\bf if} \= $(cured_i)$\\

\line{M-} \> \> {\bf then} \= $val_i \leftarrow val$;\\

\line{M-} \> \> \> $sn_i \leftarrow sn$;\\

\line{M-} \> \> \> $cured_i \leftarrow {\sf false}$;\\

\line{M-} \> \> \> {\bf for} \= {\bf each} $j \in pending\_read_i$ {\bf do}\\

\line{M-} \> \> \> \> ${\sf send}$ {\sc reply} $(i, <val_i, sn_i old\_val_i, old\_sn_i>)$;\\

\line{M-} \> \> \> \> $pending\_read_i \leftarrow pending\_read_i \setminus \{j\}$;\\

\line{M-} \> \> \> {\bf endFor}\\

%\line{M-} \> \> {\bf else} \= \\

\line{M-} \> {\bf endif}\\

\end{tabbing}
\normalsize
\end{minipage}
}
%}
% \subfigure[Write Protocol: server side]{
%\fbox{
%
%\begin{minipage}{0.4\textwidth}
% 
%% \footnotesize
%\scriptsize
% 
%\resetline
%\begin{tabbing}
%aaaA\=aA\=aA\=aaA\kill
%
%{\bf when} \=  {\sc get\_ts $(j)$} \= is  ${\sf received}$: \\ 
%
%
%
%
%\end{tabbing}
%\normalsize
%\end{minipage}
%}
%}
\caption{The state maintenance protocol for a synchronous round-free system (code for server $s_i$).}
\label{fig:stateMaintenanceProtocolRF}   
\end{figure}

%==============================================================================


%==============================================================================

\begin{figure}[t]
\centering
	\subfigure[Client code]{
\fbox{
\begin{minipage}{0.4\textwidth}
%\footnotesize
\scriptsize
%\renewcommand{\baselinestretch}{2.5}
\resetline
\begin{tabbing}
aaaA\=aA\=aA\=aaaA\kill

{\bf operation} ${\sf write}(v)$: ~~ \\

%~\\

\line{WRF-C-} \> $csn \leftarrow csn+1$;\\

\line{WRF-C-} \> ${\sf broadcast}$ {\sc write}$(v, csn)$;\\

\line{WRF-C-} \> {\bf wait} $(\delta)$;\\

\line{WRF-C-} \> {\bf return} ${\sf write\_confirmation}$;\\



\end{tabbing}
\normalsize
\end{minipage}
}
}
 \subfigure[Server code]{
\fbox{

\begin{minipage}{0.4\textwidth}
 
% \footnotesize
\scriptsize
 
\resetline
\begin{tabbing}
aaaA\=aA\=aA\=aaA\kill

{\bf when} \=  {\sc write}$(v, csn)$ \= is  ${\sf received}$: \\ 

%\line{WRF-S-} \> {\bf if} \= $(csn > sn_i)$\\

%\line{WRF-S-} \> \> {\bf then} \= $old\_val_i \leftarrow val_i$;\\
%
%\line{WRF-S-} \> \> \> $old\_sn_i \leftarrow sn_i$;\\
%
%\line{WRF-S-} \> \> \> $val_i \leftarrow v$;\\
%
%\line{WRF-S-} \> \> \> $sn_i \leftarrow csn$;\\

%\line{WRF-S-} \> \> {\bf else} \= \\

%\line{WRF-S-} \> {\bf endif}\\

\line{WRF-S-} \> $old\_val_i \leftarrow val_i$;\\

\line{WRF-S-} \> $old\_sn_i \leftarrow sn_i$;\\

\line{WRF-S-} \> $val_i \leftarrow v$;\\

\line{WRF-S-} \> $sn_i \leftarrow csn$;\\

\line{WRF-S-} \> {\bf if} \= $(cured_i)$\\

\line{WRF-S-} \> \> {\bf then} \= $cured_i \leftarrow {\sf false}$;\\

\line{M-} \> \> \> {\bf for} \= {\bf each} $j \in pending\_read_i$ {\bf do}\\

\line{M-} \> \> \> \> ${\sf send}$ {\sc reply} $(i, <val_i, sn_i, old\_val_i, old\_sn_i>)$;\\

\line{M-} \> \> \> \> $pending\_read_i \leftarrow pending\_read_i \setminus \{j\}$;\\

\line{M-} \> \> \> {\bf endFor}\\


\line{WRF-S-} \> {\bf endif}\\


\end{tabbing}
\normalsize
\end{minipage}
}
}
\caption{The ${\sf write}$ Protocol for a synchronous round-free system.}
\label{fig:writeProtocolRF}   
\end{figure}

%==============================================================================


%==============================================================================

\begin{figure}[t]
\centering
	\subfigure[Client code]{
\fbox{
\begin{minipage}{0.4\textwidth}
%\footnotesize
\scriptsize
%\renewcommand{\baselinestretch}{2.5}
\resetline
\begin{tabbing}
aaaA\=aA\=aA\=aaaA\kill

{\bf operation} ${\sf read}()$: ~~ \\

%~\\

\line{RRF-C-} \> $reply_i \leftarrow \emptyset$;\\

\line{RRF-C-} \> ${\sf broadcast}$ {\sc read}$(i)$;\\

\line{RRF-C-} \> {\bf wait }$(2\delta)$;\\

\line{RRF-C-} \> {\bf let} $<val, sn>$ be the pair occurring at least $2f+1$ times in $reply_i$;\\

\line{RRF-C-} \> {\bf return} $v$;\\


~-----------------------------------------------------------------------\\

{\bf when} \=  {\sc reply} $(j, <val, sn, oval, osn>)$ \= is  ${\sf received}$: \\ 

\line{RRF-C-} \> $reply_i \leftarrow reply_i \cup \{<j, val, sn>\}$;\\

\line{RRF-C-} \> $reply_i \leftarrow reply_i \cup \{<j, oval, osn>\}$;\\



\end{tabbing}
\normalsize
\end{minipage}
}
}
 \subfigure[Server code]{
\fbox{

\begin{minipage}{0.4\textwidth}
 
% \footnotesize
\scriptsize
 
\resetline
\begin{tabbing}
aaaA\=aA\=aA\=aaA\kill

{\bf when} \=  {\sc read} $(j)$ \= is  ${\sf received}$: \\ 

\line{RRF-S-} \> {\bf if} \= $(\neg cured_i)$\\

\line{RRF-S-} \>\> {\bf then} \= ${\sf send}$ {\sc reply} $(i, <current\_val_i, sn_i old\_val_i, old\_sn_i>)$;\\

\line{RRF-S-} \>\> {\bf else} \= $pending\_read_i \leftarrow pending\_read_i \cup \{j\}$;\\

\line{RRF-S-} \> {\bf endif}\\





\end{tabbing}
\normalsize
\end{minipage}
}
}
\caption{The ${\sf read}$ Protocol for a synchronous round-free system.}
\label{fig:readProtocolRF}   
\end{figure}

%==============================================================================

\subsection{Algorithm description}
Before to start, note that all processes start together at round $r=0$. Then clients, contrarily to the classical register implementations, do not need to compute the $timestamp$ any time that a {\sf write}() operation has to be performed.\\ 
 %just a boolean variable is enough to know if in that round we have an update value or not. If not server computes the value from the ECHOES ones.
\AD{actually just a sketch}\\
If neither a {\sf write}() or {\sf read}() operation occurs, anyway at each round servers do exchange their stored value. This is due to the fact that at each round at most $f$ servers lost their local variables (i.e. their internal state). In this situation there would not be enough servers able to correctly participate to a {\sf read}() operation. Thus for maintenance purposes at the beginning of each round servers exchange their value (line \line{}) and agree on in at the end of each round (line \line{}) considering both, the stored and the received ones.\\  
{\sf write}() operation: when a client $c_i$ wants to write a value $value$ he has just to attach to it its identifier and the current round $r$ before to broadcast $(WRITE,v)$ where $v$ is $<value, r, c_i>$ to all servers. At the server side this message will be deliver within the same round $r$. The delivered value is compared with the current stored one, if it is newer (or has a greater identifier attached) then it is stored. \\
{\sf read}() operation:  when a client $c_i$ wants to read the value stored in the register it just broadcasts $(READ)$ to all servers at round $r$. That message will be received by servers in the same round $r$ whilst the answer $(REPLY, v)$ is sent back in round $r+1$ to $c_i$. At that round $c_i$ has all the replies needed in the set variable $values$, from which it choose the one which occurs $n-2f$ times  



